Phrase-Verified Voting: Verifiable Low-Tech Remote Boardroom Voting

We present Phrase-Verified Voting, a voter-verifiable remote voting system assembled from commercial off-the-shelf software for small private elections. The system is transparent and enables each voter to verify that the tally includes their ballot selection without requiring any understanding of cryptography. This paper describes the system and its use in fall 2020, to vote remotely in promotion committees in a university. Each voter fills out a form in the cloud with their vote V (YES, NO, ABSTAIN) and a passphrase P-two words entered by the voter. The system generates a verification prompt of the (P,V) pairs and a tally of the votes, organized to help visualize how the votes add up. After the polls close, each voter verifies that this table lists their (P,V) pair and that the tally is computed correctly. The system is especially appropriate for any small group making sensitive decisions. Because the system would not prevent a coercer from demanding that their victim use a specified passphrase, it is not designed for applications where such malfeasance would be likely or go undetected. Results from 43 voters show that the system was well-accepted, performed effectively for its intended purpose, and introduced users to the concept of voter-verified elections. Compared to the commonly-used alternatives of paper ballots or voting by email, voters found the system easier to use, and that it provided greater privacy and outcome integrity.

==> notes/forms_from_google_doc.tex <==
FORMS:
\newline 
\newline 
Voting Form
Ballot for referendum REFERENDUM-ID held on DATE.
\newline
Enter two neutral words not associated with you; you might use this generator):
\newline
Enter your vote:
\newline
(checkbox selection:)
$\Box$ YES
$\Box$ NO
$\Box$  ABSTAIN
\newline
\newline 
Verification Form for Voting at Meeting
Verification of public voting data for referendum REFERENDUM-ID held on DATE.
\newline
Name: (automatically recorded)
\newline 
Select one:
(checkbox selection:)\newline 
$\Box$  I attended the meeting and voted there.
\newline
$\Box$  I attended the meeting but did not vote.
\newline
$\Box$  I attended the meeting but voted absentee.
\newline
Are your word pair and vote accurately shown?
(checkbox selection:)
\newline
$\Box$  YES
$\Box$  NO
\newline
Are the vote totals correctly shown? 
\newline That is, is it true that:
the number of votes does not exceed the number of eligible voters, and
the vote totals are correctly listed for YES, NO, and ABSTAIN ?
(checkbox selection:)
\newline
$\Box$  YES
$\Box$  NO
\newline 
\newline 
Acknowledgment Form for Absentee Voting
Verification of public voting data for referendum REFERENDUM-ID held on DATE.
\newline
Name:
(automatically recorded)
Select one: 
\newline
(checkbox selection:)
$\Box$  I voted absentee.
$\Box$  I did not vote.

==> notes/notes.tex <==
obsolete notes from early on:

\section{Protocol RBV}
\label{sec:methods}

\begin{enumerate}

\item
Rebecca publishes a list of short unique referendum descriptors (e.g., SMITH-TEACHING, SMITH-OVERALL). She also publishes a list of eligible voters.

\item
Everyone votes by sending Rebecca an email with the following information:
(B, R, V), where
B = referendum descriptor (e.g., SMITH-OVERALL),
R = eight-digit random positive integer selected by voter (e.g., 9219 7648) independently for each vote,
V = vote (e.g., one of: YES, NO, ABSTAIN).
No one votes in any other fashion (e.g., by web poll, paper, text, or phone).

\item
For each referendum, Rebecca publishes a list of the (R, V) values and a list of the eligible voters (indicating who did not vote, if any).

\item
To make a valid claim of malfeasance in a case when the claim would change the outcome, the claimant must reveal their identity, R, and V. 

\end{enumerate}

Variations:
let  $ R = h(s, V) $ to enable proof of malfeasance  in claim of changed $V$.

ideas:
 implement with Google form.
 voter may use a random number generator from web.
 would it make sense to send vote through Tor?
 Can we compel voters to verify?
 should we publish list of voters who verify?

==> notes/security_notes.tex <==
\todo[inline]{
[notes: make sure we are clear on the following.
1. trust in computers and EA.  2. MitM between voter and system.
3. computer are evil therefore your system is bad.
4. mention: software independence.  audit (not just verification).
5. security provided by Google forms (authentication of verification.
Vote only once--voter logs into Google.  Google knows how people voted.
We outsource some privacy features). also mention in trust assumptions (adversary model). complicated trust between umbc and Google, and other companies (cisco, duo) used by umbc.
6. only difference between voting and verification is that verification records identity.  Voters must be umbc but Google form doesn't check if they are eligible.
Do we stop proxy voting? A umbc person could do part, but could not verify
 To collect the names automatically on the verification form, each voter must authenticate themselves  via Google. This step deters proxy voting.
]
}

%same as note above?
%It is possible but highly unlikely that two voters pick the same $P$ value.
%Experts estimate that, with human-chosen word pairs, the chance is very small---less than 0.1\%) Experts estimate that, with human-chosen word pairs, the chance is very small (less than 0.1\%---that
%voters will select the same passphrase~\cite{}.
%Voters are welcome to use random word generators available on
%the web.\footnote{E.g., \url{https://randomwordgenerator.com/} or \url{https://www.wordgenerator.net/random-wordgenerator.php} . }
%Doing so may unnecessarily complicate the voting experience and be superfluous, and
%duplicates do not necessarily compromise outcome integrity.

\begin{comment}  %% I strongly object to the claim that "process is everything".
% This view strongly contradicts the principles of software independence and E2E: we check the OUTCOMES because we cannot assure the PROCESS.
In voting supervising and  protecting the process is everything.  When Edison brought his electric voting machine to congress, it was to inappropriately bring private voting to representatives whose constituency demanded to know how their representative voted. About the time of Edison's innovation,  people around the world started considering what Edison strived for in the congress, a private ballot.  In the 100 years since the introduction of the "Australian" private ballot, getting these ballots to reliably be deposited and counted has been the focus of voting technology.   Conflicted election officials or conspiring electorate using problems with registration procedures, voting procedures, voting place an ballot design, ballot collection, ballot counting, ballot adjudication, or ballot reporting procedures, being coerced to or volunteering to defraud elections are all problems to address. 
\end{comment}

==> notes/style_guide.tex <==

em-dash; no space around
data are



==> survey/survey.tex <==
This is the work area for creating the content of
a survey to be delivered via SurveyMonkey

What surveys should we create?
voters - yes,
election administrators (rebecca),
univ administrators? (chairs, deans, provost)
experts?
candidates?

Alternatives?
email, voice voting

should we also give to a control group (email)?

give to email dept, with video, and ask about ours?

[what we did: enabled, simplified, improved administration, made more efficient,
added security, created audit data, increased engagement?, solved chair's problem.
unified process, did this system change how voters reflected?]

[Focus first on type of information sought rather than details of how question
is worded.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Please comment on the online voting system you just used for tenure and promotion.

____
Comparing the online system versus emailing your vote:

1. How easy was it to vote?
_much worse, _slightly worse, _neutral, _slightly better, _much better

2. How much do you trust the result?
_much worse, _slightly worse, _neutral, _slightly better, _much better

3. How sure are you that your vote is private?
_much worse, _slightly worse, _neutral, _slightly better, _much better


Comparing the online system versus the in-person paper ballot voting system you used last year: 

4. How easy was it to vote?
_much worse, _slightly worse, _neutral, _slightly better, _much better
_did not use in-person voting last year

5. How much do you trust the result?
_much worse, _slightly worse, _neutral, _slightly better, _much better
_did not use in-person voting last year

6. How sure are you that your vote is private?
_much worse, _slightly worse, _neutral, _slightly better, _much better
_did not use in-person voting last year

7. What do you like and dislike about the online voting system?

8. Did the verification step increase your confidence in the result?
_not at all, _not much, _neutral, _a little bit, _a lot

9. Is the verification step worth the additional effort?
_not at all, _not much, _neutral, _a little bit, _a lot

10. Additional comments and suggestions (optional).

%%%% scratch work

Did checking your vote increase your confidence in the result?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

demographics

11. What was your role in the online voting system?
_voter, _election administrator, _university administrator

12. In what department did you participate?
_CSEE, _IS, _other:_____________________

13. Previously, have you ever used a voting system that allows voters to verify their votes?
_yes, _no

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

I. QUESTIONS FOR VOTERS (about phrase-verified voting)

The verification step was confusing.

The verification step made me feel the system was more secure.

I have confidence that my vote remained private.

What voting process did you use last year?

The voting process was too complex compared to what we used last year.

Were you familiar with verified voting systems before this fall?

I feel confident that I could use other verified voting systems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

II. QUESTIONS FOR ELECTION ADMINISTRATORS (Rebeccas)

1. What system did your unit use this fall?

2. In comparison with the system identified in (1), how would
phrase-verified voting affect the difficulty of your job in administering
tenure & promotion votes?

3. In comparison with voting -by-email, how would
phrase-verified voting affect the difficulty of your job in administering
tenure & promotion votes?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
III. QUESTIONS FOR UNIVERSITY ADMINISTRATORS (Chairs, Deans, Provost)

1. Phrase-verified voting complies with the voting system requirements
imposed by my university for tenure & promotion voting.

strongly agree
agree
neutral
disagree
strongly disagree

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

IV. QUESTIONS FOR EXPERTS

1. Compare voting-by-email with phrase-verified voting with regard to
voter usability, outcome integrity, and voter privacy.

2. Can you suggest any improvements to phrase-verified voting?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
from Ted (11-17-20)

comparing googlesheet voting with "anonymized verifiable rollcall"
with email voting

Caller of election (dean or head of department)
1. Do you think the added structure will make people vote more or less
1 less, 2 slightly less 3 same 4 more 5 much more
2. do you think the added structure will cause people to consider their decisions differently
  1 less, 2 slightly less 3 same 4 more 5 much more  
  
election administrator  
same questions
3 Do you think the structure will make your job different 
  1 easier , 2 slightly easier 3 same 4 harder  5 much harder 
  
voters
same questions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
from our initial discussions (pre 11-17-20)

1.I have been  comfortable that promotion decision voting has been done accurately in the past  

not  maybe  neutral probably absolutely
1         2            3            4           5
[intentionally laded]


2 The verification step was confusing
not  maybe  neutral probably absolutely
1         2            3            4           5
[consistent frame of ref?]

3.The verification step made me feel the system was more secure

not  maybe  neutral probably absolutely
1         2            3            4           5

4. The voting process was too complex compared to what we normally do

not  maybe  neutral probably absolutely
1         2            3            4           5


5. promotion case voting is an important part of my job
not  maybe  neutral probably absolutely
1         2            3            4           5
[what is important?  probably cut]


6. Were you familiar with verified voting systems before this fall?

7. Would you recommend that other universities use this system?

8. I would appreciate if verified voting were commonplace.

9. I feel confident that I could use other verified voting systems.


Free Form:

What did you like about phrase-verified voting?

What did you dislike about phrase-verified voting?

Additional comments (optional).

 
On Tue, Nov 3, 2020 at 2:52 PM Dr. Alan T. Sherman <sherman@umbc.edu> wrote:
We liked the general idea of questions 1-4.
We didn't like question 5 (unclear what "important" means;
unclear intent and value of question)
> I was trying to get at "do you take  this voting thing seriously" (who cares about other faculty and administration?)


6. Were you familiar with verified voting systems before this fall? 
> too leading ?   what hypothesis is this helpful for testing?
 
7. Would you recommend that other universities use this system?
> is this a  way of asking if they like it ?  
 
8. I would appreciate if verified voting were commonplace.
> again, leading 
 
9. I feel confident that I could use other verified voting systems.
> say it in a less leading way " I feel confident that this kind of system makes counting  my vote more more assured"




